Beyond Gradients: Exploiting Adversarial Priors in Model Inversion Attacks

Collaborative machine learning settings like federated learning can be susceptible to adversarial interference and attacks. One class of such attacks is termed model inversion attacks, characterised by the adversary reverse-engineering the model to extract representations and thus disclose the training data. Prior implementations of this attack typically only rely on the captured data (i.e. the shared gradients) and do not exploit the data the adversary themselves control as part of the training consortium. In this work, we propose a novel model inversion framework that builds on the foundations of gradient-based model inversion attacks, but additionally relies on matching the features and the style of the reconstructed image to data that is controlled by an adversary. Our technique outperforms existing gradient-based approaches both qualitatively and quantitatively, while still maintaining the same honest-but-curious threat model, allowing the adversary to obtain enhanced reconstructions while remaining concealed.

==> old/old_table.tex <==

\begin{table}
\centering
\caption{Activation matching (32 images, CIFAR-10, ConvNet32)}
\begin{tabular}{lccccccccc} 
\toprule
                       & \multicolumn{9}{c}{\textbf{Coefficients }}                                                                                                                                                                                                                                      \\
\multicolumn{1}{c}{}   & $s_g=1.0, s_a=1.0, s_s=0.0$ & $s_g=1.0, s_a=5.0, s_s=0.0$ & $s_g=1.0, s_a=10.0, s_s=0.0$ & $s_g=0.5, s_a=1.0, s_s=0.0$ & $s_g=0.5, s_a=5.0, s_s=0.0$ & $s_g=0.5, s_a=10.0, s_s=0.0$ & $s_g=0.1, s_a=1.0, s_s=0.0$ & $s_g=0.1, s_a=5.0, s_s=0.0$ & $s_g=0.1, s_a=10.0, s_s=0.0$  \\
MSE Difference (Mean)  &                             & 0.0188 $\downarrow$         & 0.0095 $\downarrow$          & 0.0125 $\downarrow$         & 0.0159 $\downarrow$         &                              &                             & 0.0204 $\downarrow$         & 0.0177 $\downarrow$           \\
PSNR Difference (Mean) &                             & 1.1389 $\uparrow$           & 0.3384 $\uparrow$            & 0.6117 $\uparrow$           & 0.6963 $\uparrow$           &                              &                             & 1.5508 $\uparrow$           & 1.3249 $\uparrow$             \\
SSIM Differnce (Mean)  &                             & 0.0412 $\uparrow$           & 0.0115 $\uparrow$            & 0.0192 $\uparrow$           & 0.0253 $\uparrow$           &                              &                             & 0.0579 $\uparrow$           & 0.0411 $\uparrow$             \\
\bottomrule
\end{tabular}
\label{tab:activations_mean}
\end{table}



==> tables/table_aia.tex <==
\begin{table}
\centering
\caption{Attribute inference results on the FACES dataset ($32$ images, ResNet-18).}
\resizebox{0.3\textwidth}{!}{%
\begin{tabular}{ccc} 
\toprule
                                                                & Age   & Gender attributes  \\
Inference \\performance & 22/32 & 12/32              \\
\bottomrule
\end{tabular}
}
\label{tab:aia}
\end{table}

==> tables/table_epoch.tex <==
% change to include accuracy and add the results 

\begin{table}
\centering
\caption{Attacking trained models  (32 images, various datasets, ConvNet64)}
\begin{tabular}{lcccccccc} 
\toprule
\multicolumn{1}{c}{}   & \begin{tabular}[c]{@{}c@{}}CIFAR10 \\(untrained)\end{tabular} & \begin{tabular}[c]{@{}c@{}}CIFAR10 \\(20 epochs)\end{tabular} & \begin{tabular}[c]{@{}c@{}}CIFAR10 \\(50 epochs)\end{tabular} & \begin{tabular}[c]{@{}c@{}}CIFAR10 \\(100 epochs)\end{tabular} & \begin{tabular}[c]{@{}c@{}}PPPD \\(untrained)\end{tabular} & \begin{tabular}[c]{@{}c@{}}PPPD \\(20 epochs)\end{tabular} & \begin{tabular}[c]{@{}c@{}}PPPD \\(50 epochs)\end{tabular} & \begin{tabular}[c]{@{}c@{}}PPPD \\(100 epochs)\end{tabular}  \\
MSE Difference (Mean)  & $\downarrow$   & 0.1576      & 0. $\downarrow$                                           & 0. $\downarrow$ & 0. $\downarrow$ &  0.0856    $\downarrow$                                                       & 0.0383 $\downarrow$ &  $\downarrow$                                          \\
PSNR Difference (Mean) & $\uparrow$         & 0.3437                                                              & 0 $\uparrow$                                             & 0. $\uparrow$                                              & 0. $\uparrow$                                          &     0.2063           $\uparrow$                                             & 0.0690 $\uparrow$                                          & 0. $\uparrow$                                            \\
SSIM Differnce (Mean)  & $\uparrow$      & 0.0180 & 0. $\uparrow$ & 0. $\uparrow$ & 0. $\uparrow$ & 0.0009 $\uparrow$  & 0.0011 $\uparrow$ & 0. $\uparrow$ \\
\bottomrule
\end{tabular}
\end{table}

==> tables/table_epoch_max.tex <==
% change to include accuracy and add the results 
% cifar-20 88.7%
\begin{table}
\centering
\caption{Attacking trained models  (32 images, various datasets, ConvNet64)}
\begin{tabular}{lcccccccc} 
\toprule
\multicolumn{1}{c}{}   & \begin{tabular}[c]{@{}c@{}}CIFAR10 \\(untrained)\end{tabular} & \begin{tabular}[c]{@{}c@{}}CIFAR10 \\(20 epochs)\end{tabular} & \begin{tabular}[c]{@{}c@{}}CIFAR10 \\(50 epochs)\end{tabular} & \begin{tabular}[c]{@{}c@{}}CIFAR10 \\(100 epochs)\end{tabular} & \begin{tabular}[c]{@{}c@{}}PPPD \\(untrained)\end{tabular} & \begin{tabular}[c]{@{}c@{}}PPPD \\(20 epochs)\end{tabular} & \begin{tabular}[c]{@{}c@{}}PPPD \\(50 epochs)\end{tabular} & \begin{tabular}[c]{@{}c@{}}PPPD \\(100 epochs)\end{tabular}  \\
MSE Difference (Max)  & $\downarrow$   0.6309                                          &                                                               & 0. $\downarrow$                                           & 0. $\downarrow$                                            & 0. $\downarrow$                                        &     0.2584 $\downarrow$                                                       & 0.2888 $\downarrow$                                        &  $\downarrow$                                          \\
PSNR Difference (Max) &  $\uparrow$         1.3611                                     &                                                               & 0 $\uparrow$                                             & 0. $\uparrow$                                              & 0. $\uparrow$                                          &  0.5354  $\uparrow$                                                        & 0.5329 $\uparrow$                                          & 0. $\uparrow$                                            \\
SSIM Differnce (Max)  &  $\uparrow$      0.0951                                        &                                                               & 0. $\uparrow$                                             & 0. $\uparrow$                                              & 0. $\uparrow$                                          &   0.0043  $\uparrow$                                                       & 0.0061 $\uparrow$                                          & 0. $\uparrow$                                            \\
\bottomrule
\end{tabular}
\end{table}

==> tables/table_style_max.tex <==
\begin{table*}[]
\centering
% \caption{Activation matching (32 images, CIFAR-10, ConvNet). Coefficients represent ($s_a, s_g, s_s$) respectively.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccc} 
\toprule
                       & \multicolumn{6}{c}{\textbf{Coefficients }}                                                                                                                                                       \\
\multicolumn{1}{c}{}   & (1.0, 1.0, 1.0)   & (1.0, 1.0, 100.0)     & (1.0, 1.0, 10000.0)    & (1.0, 10.0, 1.0)     & (1.0, 10.0, 100.0)     & (1.0, 10.0, 10000.0)         \\
MSE Difference (Max)  & 0.0196 $\downarrow$ & 0.0238 $\downarrow$ & 0.0532 $\downarrow$ & 0.2265 $\downarrow$ & 0.1608 $\downarrow$ & 0.1294 $\downarrow$ &   \\
PSNR Difference (Max) & 1.8618 $\uparrow$  & 1.6642 $\uparrow$   & 2.5536 $\uparrow$   & 3.6848 $\uparrow$   & 3.8306 $\uparrow$   & 2.9063 $\uparrow$   &     \\
SSIM Difference (Max)  & 0.0475 $\uparrow$   & 0.0280 $\uparrow$   & 0.0051 $\uparrow$   & 0.2791 $\uparrow$   & 0.0742 $\uparrow$   & 0.1526 $\uparrow$       \\
\bottomrule
\end{tabular}
}
\label{tab:style_max}
\end{table*}

==> tables/table_style_max_old.tex <==
\begin{table}
\centering
\caption{Style loss + activation matching (32 images, CIFAR-10, ConvNet). Coefficients represent ($s_a, s_g, s_s$) respectively.}
\begin{tabular}{lcccccccc} 
\toprule
                       & \multicolumn{8}{c}{\textbf{Coefficients }}                                                                                                                                                           \\
\multicolumn{1}{c}{}   & (1.0, 1.0, 1.0)   & (1.0, 1.0, 100.0)   & (1.0, 1.0, $10^5$.0) & (1.0, 1.0, $5 \times 10^6$.0) & (1.0, 10.0, 1.0)    & (1.0, 10.0, 100.0)  & (1.0, 10.0, $10^5$.0) & (1.0, 10.0, $5 \times 10^5$.0)  \\
MSE Difference (Max)  & VALUE $\downarrow$ & 0.0188 $\downarrow$ & 0.0095 $\downarrow$  & 0.0125 $\downarrow$           & 0.0159 $\downarrow$ & 0.0182 $\downarrow$ & 0.1078 $\downarrow$     & 0.0204 $\downarrow$             \\
PSNR Difference (Max) & VALUE $\uparrow$  & 1.1389 $\uparrow$   & 0.3384 $\uparrow$    & 0.6117 $\uparrow$             & 0.6963 $\uparrow$   & 0.7261 $\uparrow$   & 3.3312 $\uparrow$      & 1.5508 $\uparrow$               \\
SSIM Differnce (Max)  & VALUE $\uparrow$   & 0.0412 $\uparrow$   & 0.0115 $\uparrow$    & 0.0192 $\uparrow$             & 0.0253 $\uparrow$   & 0.0287 $\uparrow$   & 0.1567 $\uparrow$      & 0.0579 $\uparrow$               \\
\bottomrule
\end{tabular}
\label{ref:style_max}
\end{table}

==> tables/table_style_mean_old.tex <==
\begin{table}
\centering
\caption{Style loss + activation matching (32 images, CIFAR-10, ConvNet). Coefficients represent ($s_a, s_g, s_s$) respectively.}
\begin{tabular}{lcccccccc} 
\toprule
                       & \multicolumn{8}{c}{\textbf{Coefficients }}                                                                                                                                                           \\
\multicolumn{1}{c}{}   & (1.0, 1.0, 1.0)   & (1.0, 1.0, 100.0)   & (1.0, 1.0, $10^5$.0) & (1.0, 1.0, $5 \times 10^6$.0) & (1.0, 10.0, 1.0)    & (1.0, 10.0, 100.0)  & (1.0, 10.0, $10^5$.0) & (1.0, 10.0, $5 \times 10^6$.0)  \\
MSE Difference (Mean)  & VALUE$\downarrow$ & 0.0188 $\downarrow$ & 0.0095 $\downarrow$  & 0.0125 $\downarrow$           & 0.0159 $\downarrow$ & 0.0182 $\downarrow$ & VALUE$\downarrow$     & 0.0204 $\downarrow$             \\
PSNR Difference (Mean) & VALUE $\uparrow$  & 1.1389 $\uparrow$   & 0.3384 $\uparrow$    & 0.6117 $\uparrow$             & 0.6963 $\uparrow$   & 0.7261 $\uparrow$   & VALUE $\uparrow$      & 1.5508 $\uparrow$               \\
SSIM Differnce (Mean)  & VALUE$\uparrow$   & 0.0412 $\uparrow$   & 0.0115 $\uparrow$    & 0.0192 $\uparrow$             & 0.0253 $\uparrow$   & 0.0287 $\uparrow$   & VALUE $\uparrow$      & 0.0579 $\uparrow$               \\
\bottomrule
\end{tabular}
\label{tab:style_mean}
\end{table}
